Spatial Co-location Pattern Mining - A new perspective using Graph Database

Spatial co-location pattern mining refers to the task of discovering the group of objects or events that co-occur at many places. Extracting these patterns from spatial data is very difficult due to the complexity of spatial data types, spatial relationships, and spatial auto-correlation. These patterns have applications in domains including public safety, geo-marketing, crime prediction and ecology. Prior work focused on using the spatial join. While these approaches provide state-of-the-art results, they are very expensive to compute due to the multiway spatial join and scaling them to real-world datasets is an open problem. We address these limitations by formulating the co-location pattern discovery as a clique enumeration problem over a neighborhood graph (which is materialized using a distributed graph database). We propose three new traversal based algorithms, namely $CliqueEnum_G$, $CliqueEnum_K$ and $CliqueExtend$. We provide the empirical evidence for the effectiveness of our proposed algorithms by evaluating them for a large real-life dataset. The three algorithms allow for a trade-off between time and memory requirements and support interactive data analysis without having to recompute all the intermediate results. These attributes make our algorithms applicable to a wide range of use cases for different data sizes.

==> exp_setup.tex <==
\section{Experimental Setup}
\label{sec:ExperimentalSetup}
% \begin{figure}
% \center
% \includegraphics[width=1.0\linewidth]{fig/Architecture.pdf}
% \caption{Experimental setup architecture}
% \label{fig:Architecture}
% \end{figure}
% \begin{figure}
% \center
% \includegraphics[trim= 1cm 0cm 0cm 0cm,width=1.0\linewidth]{fig/Architecture.pdf}
% \label{fig:Architecture}
% \caption{Experimental Setup Architecture.}
% \end{figure}
%\footnote{http://thinkaurelius.github.io/titan/}
We used real world crime dataset of City of Chicago, USA \cite{dataset} for all our experiments. The data consists of crime incidents with primary crime type, address of crime incident (lat and log), date and time when crime incident occurred. We used data corresponding to 30 thousand incidents spread across 33 distinct crime types. 
\begin{figure}
\center
\includegraphics[width=0.75\linewidth]{fig/Neighbourhood_Exploration_Time_using_Titan_Standard_Indexing_and_External_Index_Elastic_New.pdf}
\caption{Neighborhood exploration time using external indexing (Elastic) and Titan standard indexing}
\label{fig:indexing}
\end{figure}
We used Titan \cite{titan}, a scalable, distributed graph database, to materialize and store the neighborhood graph. We use Titan with the Cassandra as our back-end store as most of our queries are read queries. It ensures availability, partition tolerance and eventual consistency. We partition the graph using the edge cut strategy to minimize internode communication during edge traversal. We use MongoDB as our key-value store as it supports multi-granularity locks at global, database and collection level. This level of granularity is crucial for our algorithms to execute in parallel so that the read and write operations for different candidate co-locations do not block on each other. We use Elastic \cut{\footnote{https://www.elastic.co/}} cluster to index Titan. 

% Titan supports various storage back-ends including Cassandra and HBase. Since most of our queries are read queries (traversal queries), we preferred Cassandra as our back-end store. 

% The architecture of our framework is shown in Figure \ref{fig:Architecture}. A Cassandra cluster provides the underlying storage for Titan graph database. Titan implements the Blueprint API \footnote{http://blueprints.tinkerpop.com} and exposes it to the end programmer. A MongoDB cluster is run to save co-location instances as and when required. An Elastic \footnote{https://www.elastic.co/} cluster is used to index Titan. The end application (implementation of the algorithm) uses both Titan and MongoDB. Since our entire architecture is distributed, horizontal scaling the stack is possible. 
% \\
% Notice that we use a cluster running Elastic to index Titan even though Titan comes with its own standard index. The reason is that Titan Standard Index performs good for only exact match queries while much of our queries are geo-range queries (neighborhood exploration is a geo-range query). We have compared Titan standard indexing with Elastic indexing. Figure \ref{fig:indexing} shows that neighborhood exploration time using external indexing beats Titan standard indexing as it benefits from spatial indexing. 
% \begin{figure}
% \center
% \includegraphics[width=1.0\linewidth]
% {fig/Edge_Insertion_Time_in_Titan_Graph_Using_Serial_Execution_and_Multi-threaded_Execution_New.pdf}
% \caption{Edge Insertion Time in Titan Graph Using Serial Execution and Multi-threaded Execution}
% \label{fig:result3}
% \end{figure}

In Figure \ref{fig:result3} we compare the edge insertion time using single-threaded and multi-threaded implementation. Since Elastic is distributed in nature, multi-threaded implementation beats single-threaded implementation.
Finally, we compare neighborhood exploration time in following scenarios : 
\begin{enumerate}
\item Neighborhood Exploration using Edge Traversal
\item Neighborhood Exploration using Single-threaded exectution of geo-range query
\item Neighborhood Exploration using Multi-threaded exectution of geo-range query
\end{enumerate}
We observe (Table \ref{table:neighborhood_exploration}) that edge traversal is orders of magnitude faster than both kind of geo-range query. This provides the motivation for inserting edges in the neighborhood graph instead of using geo-range queries every time.

\begin{figure}
\center
\includegraphics[width=0.75\linewidth]
{fig/Edge_Insertion_Time_in_Titan_Graph_Using_Serial_Execution_and_Multi-threaded_Execution_New.pdf}
\caption{Edge insertion time in titan graph using serial execution and multi-threaded execution}
\label{fig:result3}
\end{figure}

\begin{table}
\centering
\caption{Number of Vertices vs Neighborhood Exploration Time (in seconds) 
\label{table:neighborhood_exploration}}
\begin{tabular}{|c|c|c|c|}
\hline 
\thead{N} & \thead{Edge Traversal\\ (Single-Threaded)}  & \thead{Elastic\\(Multi-Threaded)} & \thead{Elastic\\(Single-Threaded)}\\
\hline
5000 & 0.136 & 5.307 & 298.019 \\
\hline
10000 & 0.269 & 7.484 & 1088.636 \\
\hline
15000 & 0.375 & 11.926 & 2797.643 \\
\hline
20000 & 0.494 & 16.526 & 5093.748 \\
\hline
\end{tabular}
\end{table}

